Factoring Expertise, Workload, and Turnover into Code Review Recommendation

Developer turnover is inevitable on software projects and leads to knowledge loss, a reduction in productivity, and an increase in defects. Mitigation strategies to deal with turnover tend to disrupt and increase workloads for developers. In this work, we suggest that through code review recommendation we can distribute knowledge and mitigate turnover while more evenly distributing review workload. We conduct historical analyses to understand the natural concentration of review workload and the degree of knowledge spreading that is inherent in code review. Even though review workload is highly concentrated, we show that code review natural spreads knowledge thereby reducing the files at risk to turnover. Using simulation, we evaluate existing code review recommenders and develop novel recommenders to understand their impact on the level of expertise during review, the workload of reviewers, and the files at risk to turnover. Our simulations use seeded random replacement of reviewers to allow us to compare the reviewer recommenders without the confounding variation of different reviewers being replaced for each recommender. Combining recommenders, we develop the SofiaWL recommender that suggests experts with low active review workload when none of the files under review are known by only one developer. In contrast, when knowledge is concentrated on one developer, it sends the review to other reviewers to spread knowledge. For the projects we study, we are able to globally increase expertise during reviews, +3%, reduce workload concentration, -12%, and reduce the files at risk, -28%. We make our scripts and data available in our replication package. Developers can optimize for a particular outcome measure based on the needs of their project, or use our GitHub bot to automatically balance the outcomes.

==> LetterTSE.tex <==
\textbf{Empirical RQ4, Review Workload: How is the review workload distributed across developers?}

Recent works that interview reviewers, find that experts tend to be overloaded with their review workloads~\cite{sadowski2018modern,greiler2016code} and that it is often difficult to find an available expert reviewer~\cite{greiler2016code,rigby2011understanding,thongtanunam2015should}. Before we design recommenders to balance workload, we want to understand the distribution of review effort on the projects understudy.

We replicate three studies that quantified review workload at different time scales: monthly~\cite{rigby2014peer}, weekly~\cite{kononenko2016code}, and daily~\cite{asthana2019whodo}. We find that the median reviewers performs between 2 to 4 reviews per month. The review workload on open source projects is highly skewed, with the top reviewers at the 95th percentile reviewing between 25 to 51 monthly reviews, 11 to 24 weekly reviews, and 5 to 8 daily reviews. At a quarterly level, we see that the top 20\% of reviewers accounts for an average of 80.19\% of all reviews, a clear Pareto distribution of review workload.

Dividing reviewers into core and non-core reviewers based on percentiles is reasonable for an empirical study, but does not capture the overall distribution of effort. To avoid the threshold~\cite{Mirsaeedi2020ICSE} and average-on-skewed-data~\cite{asthana2019whodo} pitfalls of prior workload measures, one of our most important contributions is a area under the cumulative distribution curve measure of workload. In this way, we capture the change in effort for both core and non-core developers in a single measure and can calculate the differences in area between recommenders to fully understand how they affect review workload.  

We note that we did not find a replication package or recommender implementation for any of these works [43].

In this section, we discuss the results for our research questions relating to (1) an empirical study of knowledge distribution during review, (2) recommendations based on ownership, including \cHRev, (3) learning and retention aware recommenders, including \sofiaEhsan, (4) an empirical quantification of the workload of reviewers, (5) recommendations based on workload, including \whodo, and a recommender that combines ownership, learning and retention, and workload, \ie \sofiaTwo.  We make three notes. First, we note that RQ1 and RQ4 do not involve simulation and are empirical result based on the actual reviews and commits. Second, we note that the MRR outcomes do not involve simulation and instead report how accurately the recommender predicts the actual reviewers. Third, simulations are run for each recommender and we note the changes in \dExpertise, \dWorkload, and \dFar as a percentage difference relative to the actual values for each project. Table~\ref{table:average} shows the average for each outcome across all projects, the values for each project are in the body of the paper.

==> intro_old.tex <==
\textbf{Empirical RQ1, Review and Turnover: What is the reduction in files at risk to turnover when both authors and reviewers are considered knowledgeable?}
%Do code reviews naturally distribute knowledge and reduce the risk of knowledge loss from developer turnover?}

Our first research question is empirical in nature and quantifies the reduction in \far from considering both authors and reviewers as knowledgeable. 
%
Recent studies have quantified knowledge loss from turnover on the basis of the commits that each developer has authored~\cite{Rigby2016ICSE,nassif2017revisiting}. 
%
However, the knowledge transfer that occurs during code review is widely documented with prior work showing that review promotes team awareness, transparency, and shared code ownership~\cite{thongtanunam2016revisiting,rigby2013convergent,sadowski2018modern,bacchelli2013expectations}. 
%
We modify the previous turnover measure to consider both authors of code as well as reviewers to be knowledgeable and recalculate the number of files that are at risk, \far.
%\peter{we need a rewrite here}
With only authors being considered knowledgeable on average 79.79\% of the total files are at risk to turnover. When we consider both authors and reviewers to be knowledgeable \far drops to 32.59\%. Code review naturally distributes knowledge.

\textbf{Simulation RQ2, Ownership Aware: Does recommending reviewers based on code and review file ownership reduce the number of files at risk to turnover?}

Studies show that teams tend to assign reviews to the owners of files under review~\cite{sadowski2018modern,greiler2016code} and experts who have modified or reviewed the files in the past~\cite{balachandran2013reducing, kovalenko2018does}. 
%
We implement ownership recommenders that suggest reviewers based on the files that developers have modified or reviewed in the past. 
%

We show that assigning reviewers based on prior commits, \authorshipRec, or prior reviews, \reviewRec, increases expertise by 10.89\% and 14.56\%, respectively, while increases turnover risk, \far, by 25.61\% and 59.65\%. For comparison purposes, we also re-implement cHRev which has been shown to outperform other recommenders~\cite{Zanjani2016TSE}. 
%
When we re-evaluate \cHRev on our outcome measures, we find that like the ownership recommenders, cHRev increases the level of expertise by 10.61\%, and has the added benefit of slightly reducing \workload by -1.72\%.
%
We conclude that concentrating expertise on the top developers make projects more susceptible to knowledge loss from turnover.

\textbf{Simulation RQ3, Turnover Aware: Can we reduce the number of files at risk to turnover by developing learning and retention aware review recommenders?}

We propose two knowledge aware proxies for estimating the degree of learning, \ie knowledge distribution, and the retention potential of each reviewer. \learnRec ensures that a developer who has not reviewed or modified all of the files currently under review will be proposed. \retentionRec recommender ensures that non-transient developers who have commitment to the project are recommended. 
%
When learning and retention factors are combined, \turnoverRec, it has the greatest reduction in turnover risk, \dFar~-29.58, with a negligible impact on \workload, 0.14\%. However, there is a substantial cost in the reduction of \expertise, -23\%

We combined awareness of ownership with learning and retention by assigns either experts or learners based on the files under review. \sofiaEhsan~\cite{Mirsaeedi2020ICSE} uses cHRev when the files under review are not at risk to turnover and uses \turnoverRec when few developers know about the files under review.
%
\sofiaEhsan increases the level of expertise during review by 6.86\%, has a negligible impact on \workload, 1.58\%, and reduces turnover risk with a \dFar of -28.83\%. 

\textbf{Empirical RQ4, Review Workload: How is the review workload distributed across developers?}

Recent works that interview reviewers, find that experts tend to be overloaded with their review workloads~\cite{sadowski2018modern,greiler2016code} and that it is often difficult to find an available expert reviewer~\cite{greiler2016code,rigby2011understanding,thongtanunam2015should}. Before we design recommenders to balance workload, we want to understand the distribution of review effort on the projects understudy.

We replicate three studies that quantified review workload at different time scales: monthly~\cite{rigby2014peer}, weekly~\cite{kononenko2016code}, and daily~\cite{asthana2019whodo}. We find that the median reviewers performs between 2 to 4 reviews per month. The review workload on open source projects is highly skewed, with the top reviewers at the 95th percentile reviewing between 25 to 51 monthly reviews, 11 to 24 weekly reviews, and 5 to 8 daily reviews. At a quarterly level, we see that the top 20\% of reviewers accounts for an average of 80.19\% of all reviews, a clear Pareto distribution of review workload. We demonstrate the concentration of review workload through an adapted Gini coefficient, \workload, and Lorenz curves. 

%Dividing reviewers into core and non-core reviewers based on percentiles is reasonable for an empirical study, but does not capture the overall distribution of effort. To avoid the threshold~\cite{Mirsaeedi2020ICSE} and average-on-skewed-data~\cite{asthana2019whodo} pitfalls of prior workload measures, one of our most important contributions is an area under the cumulative distribution curve measure of workload. In this way, we capture the change in effort for both core and non-core developers in a single measure and can calculate the differences in area between recommenders to fully understand how they affect review workload.   

\textbf{Simulation RQ5, Workload Aware: WhoDo is designed to be workload aware, but can it also balance \expertise, \workload, and \far?}

%background
In prior work, review recommenders focus on finding experts and do not measure the impact of workload~\cite{balachandran2013reducing,thongtanunam2015should,Zanjani2016TSE,xia2015should,jeong2009improving,hannebauer2016automatically}. The review recommender recently introduced at Microsoft, WhoDo, considers the ownership of prior commits and reviews and the average daily workload of each developer~\cite{asthana2019whodo}. They use the change in {\it average} workload as an outcome measure but do not consider the impact of WhoDo on \dExpertise, \dFar, or the overall distribution of workload, \dWorkload.
%what we did 
We re-implement the code for WhoDo and evaluate it in the context of open source projects on our multi-objective outcome measures. 
%result box
WhoDo increases \expertise, 7.43\%, and outperforms the existing recommenders on \workload, -11.27\%. Unfortunately, WhoDo drastically increases FaR by 45.89\% which puts many more files at risk to developer turnover.


\textbf{Simulation RQ6: Ownership, Turnover, and Workload Aware: Can we combine the recommenders to balance \expertise, \workload, and \far?}

%motivation
The ownership based recommenders are aware of the files that are recently authored or reviewed by developers (\eg cHRev~\cite{Zanjani2016TSE}), WhoDo ~\cite{asthana2019whodo} is aware of developer workload, and \sofiaEhsan~\cite{Mirsaeedi2020ICSE} is aware of files that are potentially at risk to turnover. We combine these recommenders to create a novel recommender that is aware of the ownership, workload, and knowledge distribution. When there are risky files in the pull requests we use \turnoverRec to distribute knowledge, when no files are at risk to turnover we use the \whodo recommender to find an expert developer with a low workload. 

With SofiaWorkLoad, (\sofiaTwo), \expertise is increased by 2.96\%, \workload is reduced by -12.36\%, and \far is reduced by -27.62\%. While there are recommenders that can outperform \sofiaTwo on individual outcomes only \sofiaTwo can balance all three outcomes simultaneously. 

==> more_tables.tex <==

\begin{table*}[ht]
  \centering
  \label{tab:mytable}
  \caption{Result of FaR}
  \renewcommand{\arraystretch}{1.5}
  \begin{tabular}{lccccccccc}
    \hline
    & \textbf{ChRev} & \textbf{AuthorshipRec} & \textbf{LearnRec} & \textbf{RevOwnRec} & \textbf{RetentionRec} & \textbf{TurnoverRec} & \textbf{Sofia} & \textbf{SofiaWL} & \textbf{WhoDo} \\
    \hline
    \textbf{CoreFX} & 7\% & 30\% & 27\% & 13\% & -27\% & -34\% & -32\% & -37\% & 45\% \\
    \textbf{CoreCLR} & 10\% & 11\% & 25\% & 31\% & -14\% & -12\% & -14\% & -7\% & 13\% \\
    \textbf{Roslyn} & -3\% & 35\% & 124\% & 147\% & -21\% & -41\% & -43\% & -43\% & 61\% \\
    \textbf{Rust} & 10\% & 36\% & 110\% & 100\% & -6\% & -25\% & -20\% & -20\% & 49\% \\
    \textbf{Kubernetes} & -14\% & 16\% & 72\% & 8\% & -23\% & -36\% & -35\% & -31\% & 61\% \\
    \hline
    \textbf{Average} & 9.87\% & 1.71\% & -10.66\% & -23.47\% & -16.96\% & -7.90\% & -7.88\% & 4.23\% & 45.40\% \\
    \hline
  \end{tabular}
\end{table*}

\begin{table*}
\label{tab:mytable}
  \caption{Your Table Caption Here}
  \centering
  \renewcommand{\arraystretch}{1.5}
  \begin{tabular}{lccccccccc}
    \hline
    & \textbf{ChRev} & \textbf{AuthorshipRec} & \textbf{LearnRec} & \textbf{RevOwnRec} & \textbf{RetentionRec} & \textbf{TurnoverRec} & \textbf{Sofia}  & \textbf{SofiaWL} & \textbf{WhoDo} \\
    \hline
    \textbf{CoreFX} & 10\% & 7\% & -42\% & 13\% & 14\% & -26\% & 6\% & 2\% & 6\% \\
    \textbf{CoreCLR} & 7\% & 6\% & -37\% & 10\% & 12\% & -25\% & 4\% & 0\% & 4\% \\
    \textbf{Roslyn} & 13\% & 17\% & -30\% & 19\% & 23\% & -12\% & 9\% & 4\% & 15\% \\
    \textbf{Rust} & 8\% & 11\% & -53\% & 13\% & 13\% & -34\% & 5\% & 2\% & 4\% \\
    \textbf{Kubernetes} & 14\% & 13\% & -45\% & 18\% & 20\% & -22\% & 11\% & 7\% & 8\% \\
    \hline
    \textbf{Average} & 10.61\% & 10.89\% & -41.33\% & 14.56\% & 16.37\% & -23.62\% & 6.86\% & 2.95\% & 7.43\% \\
    \hline
  \end{tabular} 
\end{table*}

